Edit Probability for Scene Text Recognition

We consider the scene text recognition problem under the attention-based encoder-decoder framework, which is the state of the art. The existing methods usually employ a frame-wise maximal likelihood loss to optimize the models. When we train the model, the misalignment between the ground truth strings and the attention's output sequences of probability distribution, which is caused by missing or superfluous characters, will confuse and mislead the training process, and consequently make the training costly and degrade the recognition accuracy. To handle this problem, we propose a novel method called edit probability (EP) for scene text recognition. EP tries to effectively estimate the probability of generating a string from the output sequence of probability distribution conditioned on the input image, while considering the possible occurrences of missing/superfluous characters. The advantage lies in that the training process can focus on the missing, superfluous and unrecognized characters, and thus the impact of the misalignment problem can be alleviated or even overcome. We conduct extensive experiments on standard benchmarks, including the IIIT-5K, Street View Text and ICDAR datasets. Experimental results show that the EP can substantially boost scene text recognition performance.

==> images/eptrie_b.tex <==
\begin{figure}[!thbp]
	\begin{center}
		\includegraphics[width=0.45\textwidth]{images/eptrie.eps}
	\end{center}
	\caption{The illustration of edit probability trie.
		The trie records a lexicon which contains three strings: ``DOVE\#'', ``DO\#'' and ``DAY\#''.
		Each node of the trie represents a prefix of one or multiple strings in the lexicon.
		Upper right to a node with the prefix $S$ is a probability vector, and the saturation of the $j$-\emph{th}(count from 0) red filled circle in the vector represents $\ep(S, A_{1:j})$ where $A$ is the output sequence of \emph{pd}.
		The higher red saturation represents the higher probability, vice versa.
	}
	\label{fig:eptrie}
\end{figure}    	

==> sections/method_b.tex <==
\section{The EP Method}\label{sec:method}
%In scene text recognition, the attention-based encoder-decoder frameworks are the state of the art. However, existing framewise-loss-based attention methods is incapable for learning dislocation problem, which may confuse the model learning process.
In this section, we present the EP method, including the formulation of EP, EP-based attention decoder, EP training, and EP predicting with/without a lexicon.

\subsection{Edit Probability}\label{sec:ep}
% definition
%Edit probability $\ep(T_{1:i} , A_{1:j})$, a mapping from $(\Sigma^*, \mathbb{R}^{|\Sigma|\times L})$ to $ [0,1]$ is the probability of generating the string prefix  $T_{1:i} \in\Sigma^*$ from the first $j$ distributions of the output sequence of probability distribution $A \in \mathbb{R}^{|\Sigma|\times L}$, where $L$ is the length of the probability distribution sequence and $T$  consists of symbols in the category set $\Sigma$.
%And the edit probability is calculated with the three types of edit operation: insertion, deletion and consumption considered.
%There are three types of operation in EP computation: insertion, deletion and consumption.
%And insertion, deletion and consumption are described in Sec. \ref{sec:intr}.
\emph{Edit probability} (EP) is proposed to effectively train attention-based models for accurate scene text recognition.
Conceptually, for an image $\mathcal{I}$ and a text string $T$, EP measures the probability of $T$ conditioned on $\mathcal{I}$ under model parameters $\theta$. It is evaluated by summing all the probabilities of edit paths that transform an initial empty string to $T$ based on the output probability distribution (\emph{pd}) sequence $A$ generated by the model. %from $\mathcal{I}$.
And each edit path consists of a sequence of edit operations which are detailed below. %, which include 1) appending a character (including the string end symbol EOS) to $S$ directly, 2) deleting the first one from the rest of the output sequence of \emph{pd} directly (if the rest is not empty), and 3) appending a character (or EOS) to $S$ by consuming the first one from the rest of the output sequence of \emph{pd} (if the rest is not empty).

\input{images/ep}

%As shown in Fig.~\ref{fig:ep}, to formally describe the calculation of EP,
Formally, let $T\in\mathbb{T}_\Sigma$ and $A\in\mathbb{P}_\Sigma^{|A|}$ where $|T|$, $|A|$, $\Sigma$, $\mathbb{T}_\Sigma$ and $\mathbb{P}_\Sigma$ represent the length of $T$, the length of $A$, the alphabet (including the EOS), the set of all valid strings (each of which contains one and only one EOS as its end token) on $\Sigma$, and the set of all probability distributions on $\Sigma$, respectively.
We define the edit statuses as tuples $(T_{1:i}, A_{1:j})$ for $0\le i\le|T|$ and $0\le j\le|A|$.
And the status $(T_{1:i}, A_{1:j})$ indicates generating $T_{1:i}$ from $A_{1:j}$.
In particular, $T_{1:0}$ and $A_{1:0}$ represent an empty string and an empty \emph{pd} sequence respectively.
By concerning the probability of the occurrence of missing/superfluous characters, the edit operations for status $(T_{1:i}, A_{1:j})$ are defined as follows:
\begin{itemize}
	%\item \emph{insertion}: an insertion operation over status $(T_{1:i}, A_{1:j})$ appends $T_{i+1}$ to $T_{1:i}$, and transforms status $(T_{1:i}, A_{1:j})$ to status $(T_{1:i+1}, A_{1:j})$ if $i<|T|$. Formally,
	\item \emph{consumption}: a consumption operation transforms status $(T_{1:i}, A_{1:j})$ to status $(T_{1:i+1}, A_{1:j+1})$ if $i<|T|$ and $j<|A|$ by regarding the character $T_{i+1}$ and the \emph{pd} $A_{j+1}$ as being correctly aligned, and
	appending $T_{i+1}$ to $T_{1:i}$ by consuming $A_{j+1}$. Formally,
	\begin{equation}
	\varepsilon^C_{i,j}(T_{1:i},A_{1:j})=(T_{1:i+1},A_{1:j+1})\text{.}
	\end{equation}
	The conditional probability of this operation is the joint probability of $R_{j+1}(1)$ and $A_{j+1}(T_{i+1})$ which respectively represent that $T_{i+1}$ is correctly aligned to $A_{j+1}$ and the classification result of $A_{j+1}$ is $T_{i+1}$. That is,
	\begin{equation}\label{eq:pc}
	p(\varepsilon^C_{i,j}|\mathcal{I};\theta)=R_{j+1}(1)A_{j+1}(T_{i+1})\text{.}
	\end{equation}
	
	\item \emph{deletion}: a deletion operation transforms status $(T_{1:i}, A_{1:j})$ to status $(T_{1:i}, A_{1:j+1})$ if $j<|A|$ by regarding the \emph{pd} $A_{j+1}$ as being superfluous, and deleting $A_{j+1}$ directly. Formally,
	\begin{equation}
		\varepsilon^D_{i,j}(T_{1:i},A_{1:j})=(T_{1:i},A_{1:j+1})\text{,}
	\end{equation}
	For $T_i\ne\text{`\#'}$, the conditional probability of this operation is $R_{j+1}(2)$ which represents that $A_{j+1}$ is superfluous. In formal:
	\begin{equation}\label{eq:pd}
		p(\varepsilon^D_{i,j}|\mathcal{I};\theta)=R_{j+1}(2)~~~\mif T_i\ne\text{`\#'}\text{.}
	\end{equation}
	And for $T_{i}=\text{`\#'}$, \emph{deletion} is the only allowed operation on status $(T_{1:i}, A_{1:j})$ as any character after the EOS is ignored. So we have
	\begin{equation}\label{eq:pd1}
		p(\varepsilon^D_{i,j}|\mathcal{I};\theta)=1~~~\mif T_i=\text{`\#'}\text{.}
	\end{equation}
	
	\item \emph{insertion}: an insertion operation transforms status $(T_{1:i}, A_{1:j})$ to status $(T_{1:i+1}, A_{1:j})$ if $i<|T|$ by regarding $T_{i+1}$ as a missing character, and appending $T_{i+1}$ to $T_{1:i}$ directly. Formally,
	\begin{equation}
	\varepsilon^I_{i,j}(T_{1:i}, A_{1:j})=(T_{1:i+1}, A_{1:j})\text{.}
	\end{equation}%. And the conditional probability of this operation %is the joint conditional probability of doing insertion and inserting the character $T_{i+1}$ before $A_{j+1}$, that is,
	For $j<|A|$, the conditional probability of this operation is the joint possibility of $R_{j+1}(3)$ and $I_{j+1}(T_{i+1})$ which respectively represent that a character is missed from the position just before $A_{j+1}$ and the missing character is $T_{i+1}$. That is,
	\begin{equation}\label{eq:pi}
	p(\varepsilon^I_{i,j}|\mathcal{I};\theta)=R_{j+1}(3)I_{j+1}(T_{j+1})~~~\mif j<|A|\text{.}
	\end{equation}
	And for $j=|A|$, \emph{insertion} is the only allowed operation over status $(T_{1:i},A_{1:|A|})$ as there is no more \emph{pd} to delete or consume. So we have \begin{equation}\label{eq:pi1}
	p(\varepsilon^I_{i,|A|}|\mathcal{I};\theta)=I_{|A|+1}(T_{j+1})~~~\mif j=|A|\text{.}
	\end{equation}
\end{itemize}
In Eq.~\ref{eq:pc}, \ref{eq:pd}, \ref{eq:pd1}, \ref{eq:pi} and \ref{eq:pi1},
%: 1) $R_j(1)$, $R_j(2)$ and $R_j(3)$ represent the probabilities that a character misses just before $A_j$, $A_j$ is superfluous, and $A_j$ is normally recognized, respectively; 2) $I_j\in\mathbb{R}^{|\Sigma|}$ represents the probability distribution of the characters (including EOS) to be inserted if the insertions are performed. While 
$R_j\in\mathbb{R}^3$ and $I_j\in\mathbb{R}^{|\Sigma|}$ are computed from the LSTM hidden state of attention, which will be described in Sec.~\ref{sec:att}. 

By assuming that the edit operations over $T$ and $A$ are conditional independent, the conditional possibility of an edit path $E$ is the joint conditional possibility of all the edit operations in $E$. That is,
\begin{equation}\label{eq:phie}
p(E|\mathcal{I};\theta)=\prod_{t=1}^{|E|} p(E_t|\mathcal{I};\theta),
\end{equation}
where $|E|$ is the length of the edit path $E$ and $E_t$ refers to the $t$-\emph{th} edit operation in $E$.
In particular, we set the conditional probability of an empty path to $1$.

The edit probability $\ep(T, A)$ is evaluated by the sum of all the conditional probabilities of edit paths $E_{1:|E|}\in\mathbb{E}_\Sigma^*$ that transform $(\text{``''}, [])$ to $(T, A)$. Formally,
\begin{equation}\label{eq:ep}
\ep(T,A)=\sum_{\substack{E\in\mathbb{E}_\Sigma^*\\E(\text{``''},[])=(T,A)}}p(E|\mathcal{I};\theta)
\end{equation}
where ``'' and $[]$ represent an empty string and an empty \emph{pd} sequence respectively, and $\mathbb{E}_\Sigma$ is the set of all edit operations over $T$ and $A$. That is,
\begin{equation}_{}\label{eq:secep}
%\begin{array}{rcl}
\mathbb{E}_\Sigma \defeq \{\varepsilon^C_{i,j}, \varepsilon^D_{i,j}, \varepsilon^I_{i,j} | 0\le i\le|T|, 0\le j\le|A|\}\text{.}
%\end{array}\text{.}
\end{equation}
%and the set of all composite edit functions on $\Sigma$. As for the composite edit function, it  is a function that recursively performs a serial of edit functions $\varepsilon$. For example, given $E = E_t \circ E_{t-1} \circ \cdots \circ E_1$, we have $E([], [])=E_t(E_{t-1}(\cdots E_1([], []) \cdots))$, where $E_t, E_{t-1}, \cdots, E_1 \in \mathbb{E}_\Sigma$ and $\circ$ represents the composite operator.
%$\phi(E):\mathbb{E}_\Sigma^*\rightarrow[0,1]$ indicates the probability of performing the composite edit function $E$ by



%In Eq.~\ref{eq:secep}, the three types of edit functions: $\varepsilon_I^k, \varepsilon_D^p, \varepsilon_C^{k, p}$ can be represented as mappings from $(\Sigma^*, \mathbb{P}_\Sigma^*)$ to $(\Sigma^*, \mathbb{P}_\Sigma^*)$:
%\begin{equation}
%\left\{\begin{array}{rcl}
%\varepsilon_I^k(T_{1:i},A_{1:j}) &=& (T_{1:i}\oplus k,A_{1:j})\\
%\varepsilon_D^p(T_{1:i},A_{1:j}) &=& (T_{1:i},A_{1:j} \oplus  p)\\
%\varepsilon_C^{k,p}(T_{1:i},A_{1:j}) &=& (T_{1:i}\oplus k,A_{1:j}\oplus p)
%\end{array}\right.\text{,}
%\end{equation}
%where $\oplus$ means the concatenation operation between two  sequences.

%%%%%%%%%%%%%%%%%%%%% Fan Bai %%%%%%%%%%%%%%%%%%
%Edit Probability $\ep(T , A):(\Sigma^*, \mathbb{R}^{|\Sigma|\times L})\rightarrow [0,1]$ is the probability of generating sequences with prefix $T$ conditioned on the given probability distribution sequence $A_{|\Sigma|\times L}$ with insertions, deletions and consumptions taken into account,
%where $L$ is the length of the probability distribution sequence and $T$  consists of symbols in the category set $\Sigma$.
%There are three types of operation in EP computation: insertion, deletion and consumption, and Eq. \ref{sec:intr} describes the operations.
%Insertion and deletion are like what described in \ref{sec:intr}.
%And consumption means a pair of distribution and unit in the distribution sequence and the result sequence are considered as matched(\eg $A_j$ and $T_i$),
%and the probability of $T_i$ in $A_j$ is ``consumed'' to generate $T_i$ where $A_j$ means the $j$-th column of $A$.

%The character sequence generation from $A$ can be carried out with a sequence of steps.
%For example, given the generated prefix  $T_{1:i}\in\Sigma^i$   from the first $j$ probability distribution $A_{1:j} \in \mathbb{R}^{j\times |\Sigma|}$, we can perform the following edit operations in the next step:

%%%%%%%%%%%%%%%%%%%%% Fan Bai %%%%%%%%%%%%%%%%%%
%The process of transforming $A$ to a result sequence can be divided into a sequence of steps.
%On the status we have produced $S\in\Sigma^*$ from $A_{1:j}$, we can perform the following edit operations in the next step:
%\begin{itemize}
%        	\item inserting a unit $k$ back to $S$ (if we believe a incorrect deletion occurs), denoted by edit function $\varepsilon_I^k$ where $k\in\Sigma$;
%        	\item deleting the next probability distribution $p$ with $S$ unchanged (if we believe a incorrect insertion occurs), denoted by edit function $\varepsilon_D^p$, where $p=A_{j+1}\in \mathbb{P}_\Sigma$ is a probability distribution on category set $\Sigma$, $\mathbb{P}_\Sigma\subset\mathbb{R}^{|\Sigma|}$ is the set of distributions on category set $\Sigma$ and
%        	\begin{equation}
%        		\forall p\in\mathbb{P}_\Sigma, \sum_{k\in\Sigma}p(k)=1\text{;}
%        	\end{equation}
%        	\item generating a symbol $k$ back to $S$ by consuming the next possibility distribution $p$ (if we believe that $p$ matches this symbol $k$), denoted by edit function $\varepsilon_C^{k, p}$, where $k\in\Sigma$ and $p=A_{j+1}\in\mathbb{P}_\Sigma$.
%        \end{itemize}
%Formally, we define $\mathbb{E}_\Sigma$ as the set of all edit functions on $\Sigma$:

% dp
However, enumerating all the possible edit path is prohibitively expensive even impossible as the search space is too large.
Fortunately, this can be solved by dynamic programming based on the following equation inferred from Eq.~\ref{eq:phie}:
        \begin{equation}\label{eq:phi1}
		        p(\varepsilon \circ E^\prime|\mathcal{I};\theta) = p(E^\prime|\mathcal{I};\theta)p(\varepsilon|\mathcal{I};\theta)\text{,}
        \end{equation}
%{\color{red}because performing $E_1$ and $\varepsilon$ is independent}
where $\varepsilon$, $E^\prime$ and $\circ$ represent an edit operation, an edit path, and the concatenation operator for two edit paths, respectively. The concatenation operator for two edit paths is defined as follows:
\begin{equation}
	(E_2\circ E_1)(T_{1:i},A_{1:j})=E_2(E_1(T_{1:i},A_{1:j}))
\end{equation}
where both $E_1$ and $E_2$ are edit paths or operations.
%Similar to the forward-backward algorithm in CTC~\cite{alex06ctc}, the core idea is that the edit probability of a certain edit status can be computed from the edit probabilities of some other statuses that can be transformed to the former status with one edit operation. 
With Eq.~\ref{eq:phi1}, we can rewrite Eq.~\ref{eq:ep} as follows:
\begingroup
\renewcommand*{\arraystretch}{1.24}
        \begin{equation}\label{eq:eprewrite}
            \begin{array}{rl}
                &\ep(T_{1:i},A_{1:j})\\
                =&\sum\limits_{\substack{E^\prime \in \mathbb{E}_{\Sigma}^*, \varepsilon \in \mathbb{E}_{\Sigma}  \\ \varepsilon(E^\prime(\text{``''},[]))=(T_{1:i},A_{1:j})}} p(E^\prime|\mathcal{I};\theta)p(\varepsilon|\mathcal{I};\theta) \\
               =& \sum\limits_{\substack{\varepsilon \in \mathbb{E}_\Sigma  \\   (T^\prime, A^\prime) \in (\mathbb{T}_\Sigma, \mathbb{P}_{\Sigma}^*) \\ \varepsilon(T^\prime, A^\prime)=(T,A) }} p(\varepsilon|\mathcal{I};\theta)
                         \sum\limits_{\substack{E^\prime \in \mathbb{E}_{\Sigma}^*  \\ E^\prime(\text{``''},[])=(T^\prime,A^\prime)}} p(E^\prime|\mathcal{I};\theta) \\
               =& \sum\limits_{\substack{\varepsilon \in \mathbb{E}_\Sigma^*  \\   (T^\prime, A^\prime) \in (\mathbb{T}_\Sigma, \mathbb{P}_{\Sigma}^*) \\ \varepsilon(T^\prime, A^\prime)=(T,A) }} p(\varepsilon|\mathcal{I};\theta) \ep(T^\prime, A^\prime)\\
               =&\left\{
               	        \begin{array}{lr}
               		        \multicolumn2l{1 \hspace{42mm} \mif i=0, j=0}\\
%               		        {\ep(T_{1:i},A_{1:j-1})R_j(2)} &
%               		        {\mif i=0, j>0} \\
%               		        {\ep(T_{1:i-1},A_{1:j})R_j(3)I_j(T_i)}&
%               		        {\mif i>0, j=0} \\
%               		        {\ep(T_{1:i},A_{1:j-1})R_{j+1}(2)}&{\mif i>0, j>0,} \\
%               		         \multicolumn2l{~~ +\ep(T_{1:i-1},A_{1:j})R_j(3)I_j(T_i)~~~\text{and~}T_{i}\ne\text{`\#'}}\\
%               		         \multicolumn2l{~~ +\ep(T_{1:i-1},A_{1:j-1})R_j(1)A_j(T_i) } \\
%               		         {\ep(T_{1:i},A_{1:j-1})}  & {\mif i>0, j>0,} \\
%               		         \multicolumn2l{~~ +\ep(T_{1:i-1},A_{1:j})R_j(3)I_j(T_i)~~~\text{and~}T_{i}=\text{`\#'}}\\
%               		         \multicolumn2l{~~ +\ep(T_{1:i-1},A_{1:j-1})R_j(1)A_j(T_i) } \text{.}\\
               		         \ep(T_{1:i},A_{1:j-1})\delta_{T_i=\text{`\#'},j>0} & \text{otherwise}\\
               		         \multicolumn2l{~~ +\ep(T_{1:i},A_{1:j-1})R_j(2)\delta_{T_i\ne\text{`\#'},j>0}}\\
               		         \multicolumn2l{~~ +\ep(T_{1:i-1},A_{1:j})I_j(T_i)\delta_{i>0,j=|A|}}\\
               		         \multicolumn2l{~~ +\ep(T_{1:i-1},A_{1:j})R_j(3)I_j(T_i)\delta_{i>0,j<|A|}}\\
               		         \multicolumn2l{~~ +\ep(T_{1:i-1},A_{1:j-1})R_j(1)A_j(T_i)\delta_{i>0,j>0}}
               	        \end{array}
               	        \right.
		        %\text{.}
             \end{array}
        \end{equation}
\endgroup
where the value of $\delta_{condition}$ is $1$ if the condition is met, otherwise $0$.
By recursively applying Eq.~\ref{eq:eprewrite}, $\ep(T, A)$ can be calculated in $O(|T|\cdot|A|)$.

Fig.~\ref{fig:ep} shows the calculation of EP for generating ``DOVE\#'' from the sequence of \emph{pd} displayed in Fig.~\ref{fig:mot}~(a). We can see that an insertion operation which inserts an `O' is contained in the maximal probable edit path, which is as expected.

%In the following, in order to facilitate the description of this dynamic programming algorithm, we call the elements of $(\Sigma^*, \mathbb{P}_{\Sigma}^*)$ \textit{status}. And for a particular status $(T_{1:i}, A_{1:j})$:
%\begin{itemize}
%  \item If $i=0, j=0$, that is, $T_{1:i}=[]$ and $A_{1:j}=[]$, it cannot be a result of any edit operation. And we define
%              \begin{equation}\label{eq:tab1}
%    		        \ep(T_{1:0}, A_{1:0}) = \ep([], []) =  1
%              \end{equation}
%  \item For $i=0, j>0$, it must be the result of a deletion operation. We have
%              \begin{equation}\label{eq:tab2}
%    		        \ep([], A_{1:j}) = \ep([], A_{1:j-1})\phi(\varepsilon_D^{A_j})
%              \end{equation}
%  \item For $i>0, j=0$, it must be the result of a insertion operation. We have
%              \begin{equation}\label{eq:tab3}
%    		        \ep(T_{1:i}, []) = \ep(T_{1:i-1}, [])\phi(\varepsilon_I^{T_i})
%              \end{equation}
%  \item For $i>0, j>0$, it can be the result of any of the three kinds of edit operations. We have
%              \begin{equation}\label{eq:tab4}
%                    \begin{array}{l}
%    		              \ep(T_{1:i}, A_{1:j}) = \ep(T_{1:i-1},A_{1:j})\phi(\varepsilon_I^{T_i}) \\
%                                        ~~~~~~~~~~~~~~~~                                +   \ep(T_{1:i},A_{1:j-1}) \phi(\varepsilon_D^{A_j}) \\
%                                        ~~~~~~~~~~~~~~~~                          +  \ep(T_{1:i-1},A_{1:j-1}) \phi(\varepsilon_C^{T_i, A_j}).
%                    \end{array}
%              \end{equation}
%\end{itemize}

%Concretely, the computation of $\phi(\varepsilon): \varepsilon \in \mathbb{E}_\Sigma$ depends on the probability distribution $P_w\in \mathbb{R}^3$ on performing three types of edit operations: insertion probability $P_I$, deletion probability $P_D$ and consumption probability $P_A$.
%And $P_w$ is calculated by:
%        \begin{equation}
%            P_w = [P_I, P_D, P_C] = softmax(WA_f + \omega)\text{,}
%        \end{equation}
%where $W\in \mathbb{R}^{3 \times |\Sigma|  L}$ and $\omega \in \mathbb{R}^{3}$ are trainable parameters, and $A_f \in \mathbb{R}^{|\Sigma|L} = flatten(A)$.
%Particulary,
%\begin{itemize}
%  \item If the insertion operation is performed, the probability of inserting a particular character $k$ is denoted as $I(k): k\in\Sigma$, and
%            \begin{equation}
%                    	I =  softmax(UA_f + \mu)\text{,}
%            \end{equation}
%            where $U\in \mathbb{R}^{|\Sigma| \times |\Sigma|  L}$ and $\mu \in \mathbb{R}^{\Sigma}$ are trainable parameters, and $I\in\mathbb{R}^{|\Sigma|}$.
%  \item For consumption operation, the probability of generating a particular character $k$ is denoted as $p(k):k\in\Sigma$ by directly consuming the distribution $p$.
%  \item For deletion operation,  the next probability distribution $p$ is directly deleted.
%\end{itemize}
%Then $\phi(\varepsilon)$ can be represented as:
%        \begin{equation}\label{eq:phi0}
%        	\left\{\begin{array}{rcl}
%        		\phi(\varepsilon_I^k) &=& P_II(k)\\
%        		\phi(\varepsilon_D) &=& P_D\\
%        		\phi(\varepsilon_C^{k,p}) &=& P_Cp(k)
%        	\end{array}\right.\text{.}
%        \end{equation}

%With Eq.~\ref{eq:eprewrite} $\sim$  \ref{eq:tab4} and \ref{eq:phi0}, we have
%%Substituting Eq.~\ref{eq:phi0} and Eq.~\ref{eq:phi1} into Eq.~\ref{eq:ep}, $\ep(T, A)$ can be calculated, shown in Fig.~\ref{fig:ep} (a), with dynamic programing algorithm Eq.~\ref{eq:epdp}:
%        \begin{equation}\label{eq:epdp}
%	        \ep(T_{1:i},A_{1:j})=\left\{
%	        \begin{array}{lr}
%		        1 & \mif i=1, j=1\\
%		        \multicolumn2l{\ep(T_{1:i},A_{1:j-1}) P_D} \\
%		        \multicolumn2r{\mif i=1, j\ne 1} \\
%		        \multicolumn2l{\ep(T_{1:i-1},A_{1:j}) P_I I(T_i)} \\
%		        \multicolumn2r{\mif i>1, j=1} \\
%		         \multicolumn2l{\ep(T_{1:i-1},A_{1:j}) P_I I(T_i)} \\
%		         \multicolumn2l{~~ +\ep(T_{1:i},A_{1:j-1}) P_D} \\
%		         \multicolumn2l{~~ +\ep(T_{1:i-1},A_{1:j-1}) P_C A_{j,T_i} } \\
%		         \multicolumn2r{\mif i>1, j>1} \\
%	        \end{array}
%	        \right.
%        \end{equation}
%As shown in figure \ref{fig:ep} (a), $\ep(T, A)$ can be calculated with dynamic programing algorithm Eq.~\ref{eq:epdp}.


%Besides, the sequence recognition task needs to generate sequences of variable lengths.
%Similar to attention-based methods[][][][], we also add an end-of-sequence symbol $EOS$ (\#)  into the category set $\Sigma$.
%n other word,  extra characters should not be appeared after an $EOS$ in a sequence.
%As generating the prefix $T\oplus\#$ is equivalent to generate the complete sequence $T\oplus\#$, we have
%And the likelihood $\p(T|A)$  is equivalent to $\ep(T\oplus EOS, A)$:
%{\color{red}In other word, $\p(T|A)$  is equivalent to $\ep(T\oplus EOS, A)$ due to $EOS \notin T$}:
%    	\begin{equation}\label{eq:ep2}
%    		\p(T|A) = \ep(T\oplus \#,A)
%    	\end{equation}
%where $\p(T|A)$ is the likelihood of $T$ conditioned on A.

%{\color{red}
%Note that,
%}
%Eq.~\ref{eq:tab4} is suit for the cases without $EOS$. For  $T_{1:i-1}\oplus EOS$ ($EOS\not\in T_{1:i-1}$), we have
%\begin{equation}\label{eq:tab42}
%\begin{array}{l}
%\ep(T_{1:i-1}\oplus \#, A_{1:j}) = \ep(T_{1:i-1},A_{1:j})\phi(\varepsilon_I^{\#}) \\
%~~~~~~~~~~~~~~~~                                +   \ep(T_{1:i-1}\oplus \#,A_{1:j-1}) \\
%~~~~~~~~~~~~~~~~                          +  \ep(T_{1:i-1},A_{1:j-1}) \phi(\varepsilon_C^{\#, A_j}).
%\end{array}
%\end{equation}
%because any insertion and consumption edit function after an $EOS$  is not allowed to be performed (as they cause extra characters after $EOS$),  while the deletion edit operation is the only one allowed to be performed.

%Fig.~\ref{fig:ep} (b) depicts the calculation of $ \ep(T\oplus \#,A)$.

%{\color{red}
%Considered the insertion deletion operations, the $ \ep(T\oplus EOS,A)$ is a better way to {\color{red}describe} character sequences generation than the CE or CTC.
%}

\subsection{EP-based Attention Decoder}\label{sec:att}
The classic attention decoder is an RNN which generates the output \emph{pd} $A_j$ on the $j$-\emph{th} step\cite{bahdanau2016end}:
\begingroup
\renewcommand*{\arraystretch}{1.4}
\begin{equation}\label{eq:att}
\begin{array}{rcl}
	A_j &=& \softmax(W_A^\top s_j),\\
	s_j &=& \LSTM(y_{j-1}, c_j, s_{j-1}),\\
	c_j &=& \sum_{k^\prime=1}^{|h|}\alpha_{j,k}h_k,\\
	\alpha_{j,k} &=& \dfrac{\exp(e_{j,k})}{\sum_{k^\prime=1}^{|h|}\exp(e_{j,k})},\\
	e_{j,k} &=& w^\top\tanh(Ws_{j-1}+Vh_{k}+b)
\end{array}
\end{equation}
\endgroup
where $h$ is a sequence of encoded feature vector, and $s_j$, $c_j$, $\alpha_j$ and $e_j$ represent the LSTM~\cite{hochreiter97lstm} hidden state, the weighted sum of $h$, the the attention weights and the alignment model on the $j$-\emph{th} step, respectively.
Above, $w$, $W$, $V$, $b$ and $W_A$ are all trainable parameters.
%$g_A$ and $f$ represent a feed-forward network and an LSTM recurrent network, respectively.

In this work, to satisfy the EP calculation, the attention decoder also generates $R_j$ and $I_j$ on the $j$-\emph{th} step:
\begingroup
\renewcommand*{\arraystretch}{1.25}
\begin{equation}
\begin{array}{rcl}
R_j &=& \softmax(W_R^\top s_j),\\
I_j &=& \softmax(W_I^\top s_j)
\end{array}
\end{equation}
\endgroup
where $W_R$ and $W_I$ are also trainable parameters.
Note that, an extra step of attention is required in order to generate $I_{|A|+1}$ for Eq.~\ref{eq:pi1}.
\subsection{EP Training}
With the training set $\mathcal{X}$ which consists of pairs of image and \emph{gt} string, the EP-based model is trained to minimize the negative log-likelihood over $\mathcal{X}$, that is, to minimize the following
%The aim of maximum likelihood training is to minimize the negative log-probabilities of all the ground truth sequence conditioned on the corresponding input data in the training set. For a particular training image $\mathcal{I}$, that is, to minimize $\p(T', A)$ where the character sequence $T'$ is the ground truth and the sequence of probability distribution $A$ is the output of the sequence-recognition-based neural network with input $\mathcal{I}$.
objective function:
		\begin{equation}\label{epl}
			J=-\sum_{(\mathcal{I},T^\prime)\in\mathcal{X}}\ln(\ep(T^\prime, A))
		\end{equation}
where $A$ is the output sequence of \emph{pd} conditioned on $\mathcal{I}$ under model parameters $\theta$ and is computed by Eq.~\ref{eq:att}, while $\ep(T^\prime, A)$ is edit probability of edit status $(T^\prime, A)$ defined in Eq.~\ref{eq:ep} and computed by Eq.~\ref{eq:eprewrite}.
%where $T^\prime$ is the ground truth.
The model can be optimize with standard back-propagation algorithm\cite{rumelhart1988learning}.


\subsection{EP Predicting}\label{sec:epp}
EP Predicting is to find the string $\hat{T}$ which maximize $\ep(\hat{T}, A)$ where A is the output sequence of \emph{pd} conditioned on the input data $\mathcal{I}$:%, that is, to find the prefix sequence $\hat{T}\oplus EOS$ which equals to maximize the probability conditioned on the distribution sequence $A$:
    	\begin{equation}\label{eq:epp}
    		\hat{T} = \arg\max_{\tilde{T}\in{\mathbb{T}_\Sigma}}\ep(\tilde{T}, A)\text{.}
    	\end{equation}
However, looking for the whole answer set ${\mathbb{T}_\Sigma}$ with Eq. \ref{eq:epp} is extremely costly, even impossible.
Therefore, we develop two efficient sequence generation mechanisms for both lexicon-free and lexicon-based prediction.
    	
\textbf{Predicting without lexicon.}
%In general, for a well trained model,  the character sequences with the largest edit probability are more probably generated by directly consuming each probability of $A$.
%Therefore, instead of looking for the whole answer set $\Sigma^*$, we define a candidate set $\mathcal{B}_A$ based on $A$ as following:
 %   	\begin{equation}\label{eq:cand}
  %          \mathcal{B}_A=\pref(\max A_1 \oplus \max A_2  \oplus \cdots  \oplus A_{L-1})
   % 		%\mathcal{B}_A=\pref(\sum_{i=1}^{L-1}\max_{k\in\Sigma-EOS}A_i(k))
%    	\end{equation}
%where $\pref(S)$ means the set of $S$'s prefixes.
%For example,  given $A$ in Fig. \ref{fig:mot}$ (a), \mathcal{B}_A$ consists of ``'', ``A'', ``AC'', ``ACD'', ``ACDD'' and ``ACDDD''.
%Note that, the $EOS$ ($\#$) is removed.
%For each $\tilde{T}\in\mathcal{B}_A$, $\ep(\tilde{T} \oplus EOS, A)$ is lexicographically calculated in O($L$) with Eq. \ref{eq:ep}.
%Finally, we select the one with the maximal probability generated from $A$ as the predicted result:
%    	\begin{equation}\label{eq:eplp}
%    		\hat{T} = \max_{\tilde{T}\in\mathcal{B}_A}\ep(\tilde{T} \oplus EOS, A)\text{.}
 %   	\end{equation}
 %After carefully observation and analysis
 After a lot of investigation, we find that in general,
 %{\color{red}
 the string $\hat{T}$ who maximizes $\ep(\hat{T},A)$  is mostly a prefix(with an EOS appended at the end) of the string $\mathcal{T}$ with the most probable edit path which transforms $(\text{``'',[]})$ to $(\mathcal{T}, A)$, and $\text{`\#'}\not\in\mathcal{T}$.

 Therefore, we firstly find the string $\mathcal{T}$:
  \begin{equation}\label{eq:T}
 %\arg\max_{\tilde{T}\in\Sigma^*}\ep(\tilde{T}+EOS, A) =
 	\mathcal{T} = \arg\max_{\tilde{T}\in(\Sigma\backslash\{\text{`\#'}\})^*}\max_{\substack{E\in\mathbb{E}_{\Sigma}^*\\E(\text{``''},[])=(\tilde{T}, A)}}p(E|\mathcal{I};\theta)
 \end{equation}
 where $\Sigma\backslash\{\text{`\#'}\}$ represents the alphabet without the EOS,
 then use all the prefixes of $\mathcal{T}$(with an EOS appended at the end) as the candidate set $\mathcal{B}$:
 \begin{equation}\label{eq:cand}
	\mathcal{B} = \{\mathcal{T}_{1:i}\oplus\text{`\#'}|0\le i\le|\mathcal{T}|\}
 \end{equation}
 where $\oplus$ represents the concatenation operator for two strings,
 finally select the best $\hat{T}\in\mathcal{B}$ which maximizes $\ep(\hat{T}, A)$:
  \begin{equation}\label{eq:cand}
 	\hat{T} = \arg\max_{\tilde{T}\in\mathcal{B}}\ep(\tilde{T}, A)\text{.}
 \end{equation}


 %{\color{red}
Note that, the edit path with the highest probability should not include an insertion edit operation which inserts a non-EOS character,
because
%$(E_2\circ\varepsilon^I_{i,j}\circ E_1)([],[])=(T_1\oplus T_2, A) \Rightarrow(E_2\circ E_2)([],[])=(T_1\oplus T_2, A)$
%while
%$p(E_2\circ\varepsilon_I^k\circ E_2) = p(E_2\circ E_2|\mathcal{I};\theta)p(\varepsilon^I_{i,j}|\mathcal{I};\theta) \le p(E_2\circ E_2|\mathcal{I};\theta)$.
we can remove all the insertions in the edit path and get a new edit path whose conditional probability is greater than the previous one's.

Therefore, we can generate $\mathcal{T}$ by beginning at the status $(\text{``''},[])$ and performing the most probable operation in deletions and consumptions~(excluding the one generates the EOS) on each step, until reach a status $(\mathcal{T}, A)$. And since the strings in $\mathcal{B}$ share the common prefixes, we can compute all the $\ep(\tilde{T}, A)$ for $\tilde{T}\in\mathcal{B}$ in $O(|\mathcal{T}|\cdot|A|)$ time with Eq.~\ref{eq:eprewrite}.
%\begin{equation}
%\begin{array}{lcr}
%	\mathcal{T} &\defeq& \mathcal{T}_{A}\\
%	\mathcal{T}_{A_{1:j}}&=&\left\{\begin{array}{lr}
%		\mathcal{T}_{A_{1:j}} &\\
%		\mathcal{T}_{A_{1:j}}\oplus &
%	\end{array}\right.\\
%	\mathcal{T}_{A_{1:0}}&=&\text{``''}
%\end{array}
%\end{equation}
%from status $(\text{``''}, [])$, and on each status $(T_{1:i}, A_{1:j})$, we separately perform:
%\begin{itemize}
%	\item ending the string with appending an $EOS$ directly or by consuming the $A_{j+1}$(if $j<|A|$), then add the string into the candidate set $\mathcal{B}_A$;
%	\item select the highest possible edit operation from deletion or consumptions (generating any character except for $\#$ by consuming the next probability distribution), then perform it.
%	%}
%\end{itemize}
%Finally, we select the one with the maximal edit probability generated from $A$ as the predicted result:
%    \begin{equation}\label{eq:eplp}
%    		\hat{T} = \arg\max_{\tilde{T}\in\mathcal{B}_A}\ep(\tilde{T} \oplus EOS, A)\text{.}
%   	\end{equation}
    	
    	
\input{images/eptrie}
    	
\textbf{Predicting with a lexicon.}\label{sec:pwl}
In constrained case, we  can enumerate the strings in a lexicon $\mathcal{D}$, and find the most probable one.
And a tunable parameter $\lambda$ is used to indicate how much we trust the lexicon $\mathcal{D}$ since some target string may be not contained in the lexicon.
Therefore we actually appraise all the possible strings in $\mathcal{B} \cup \mathcal{D}$ by
    	\begin{equation}
    		\hat{T} = \arg\max_{\tilde{T}\in\mathcal{B}\cup\mathcal{D}}\left\{
    		\begin{array}{lr}
    			\lambda\ep(\tilde{T}, A) & \mif \tilde{T}\in\mathcal{D}\\
    			(1-\lambda)\ep(\tilde{T}, A) & \mif \tilde{T}\not\in\mathcal{D}
    		\end{array}
    		\right.
    	\end{equation}
where $0.5\le\lambda\le1$.
The larger $\lambda$ is, the more we trust the lexicon, vice versa.
Specially, $\lambda=0.5$ means that the lexicon only provides some more candidates which are treated equally to those in $\mathcal{B}$, while $\lambda=1$ means that the generated string is guaranteed to appear in the lexicon $\mathcal{D}$.
    	

	
However, with the growing of the lexicon size, the above enumeration-based method is extremely time-consuming.
To tackle this problem, Shi \etal first use a prefix tree(also called trie)\cite{briandais1959trie,shi2016robust} to accelerate the searching process since many strings in the lexicon share common prefixes.
As shown in Fig.~\ref{fig:eptrie}, in this case, we develop a data structure called \textbf{edit probability trie (EP-Trie)} which is a variant of trie with nodes containing not only a prefix $S$,
but also a vector indicating $\ep(S, A_{1:j})$ for $0\le j\le|A|$.
And each vector of a node can be computed from the vector of its parent node in O($|A|$) time with Eq. \ref{eq:eprewrite}.
Finally, we demonstrate the effectiveness of acceleration of EP-trie in Sec. \ref{sec:dop}.

==> sections/related_b.tex <==
%------------------------------------------------------------------------
\section{Related work}\label{sec:related-work}
%------------------------------------------------------------------------
% current loss
%At the present stage, most of encoder-decoder frameworks are trained with Cross Entropy Loss [] or CTC Loss.
%However, both of CE and CTC can not tackle with incorrect insertions and deletions in the output probability distribution sequence well.
% CE loss
%The CE calculates cross entropy between the sequence of ground truth and the output sequence column by column, but it does not take into account contextual relationships.
% CTC loss
%The Connectionist Temporal Classification is another popular technique for mapping the encoded sequences to target sequences, but it only considers incorrect insertions.
% EP
%In order to consider both insertions and deletions in sequence generation, we design the EP to capture the target deleting or inserting probability.

%In scene text recognition tasks, the encoder-decoder-based sequence recognition framework has been wildly used in previous works[][][][][].
%We find that most of encoder-decoder frameworks are trained with Cross Entropy Loss [] or CTC Loss.
%The CE-based methods calculates cross entropy as the loss between the sequence of ground truth and the output sequence column by column, but it does not take into account contextual relationships. While the CTC-based methods calculate loss by mapping the encoded sequences to target sequences, but it only considers incorrect insertions.

% background
In the past decade, many methods have been proposed for scene text recognition, which roughly fall into three types: 1) traditional with handcrafted features, 2) Na\"ive deep neural-network-based, and 3) sequence-based.

% traditional methods
In early years, traditional methods first extract handcrafted visual features for individual character detection and recognition one by one, then integrate these characters into words based on a set of heuristic rules or a language model.
Neumann and Matas~\cite{neumann2012real} recognized characters by training a Support Vector Machine (SVM) classifier with the defined handcrafted features such as aspect ratio, hole area ratio etc. Wang \etal~\cite{wang2011end,wang2010word} first trained a character classifier with the extracted HOG descriptors~\cite{yao2014strokelets}, then recognized characters of the cropped word image by a sliding window one by one.
However, the low representation capability of handcrafted features limits the recognition performance.

% cnn-based methods
Later, instead of handcrafted features, some deep neural-network-based methods were developed for extracting robust visual features.
Bissacco \etal~\cite{bissacco2013photoocr} adopted a fully connected network (FC) of 5 hidden layers for extracting character features, then applied an n-gram language model to recognize characters.
Wang \etal~\cite{wang2012end} and Jaderberg \etal~\cite{jaderberg2014deep, jaderberg2016reading} first developed CNN-based framework for character feature representation, then applied some heuristic rules for characters generation.
These na\"ive deep neural-network-based methods above usually recognized character sequence based on some pre/post-processing, such as the segmentation of each character or a non-maximum suppression, which may be very challenging due to the complicated background and the inadequate distance between consecutive characters.

% sequence-based methods
Recently, some researchers treated the text reading task as a sequence recognition problem: first encoding a text image into a sequence of features with deep neural network, then directly generating character sequence with sequence recognition techniques.
He \etal~\cite{he2016deep}, Shi~\etal\cite{shi17end} proposed the end-to-end neural networks that first capture visual feature representation by using CNN or RNN, then the CTC~\cite{alex06ctc} loss was combined with the neural network outputs for calculating the conditional probability between the predicted and the target sequences.
The state of the art for text reading is the attention-based methods~\cite{cheng17fan,lee16recursive,shi2016robust}. %Yang \etal [],
%A latest such method was proposed by Cheng \etal~\cite{2017arXiv170902054C}.
These methods first combined CNN and RNN for encoding text images into feature representation, then employed a framewise loss to optimize the model. In the training process, the misalignment between the $gt$ sequence and the output $pd$ sequence may mislead the training algorithm and result in poor performance.

Note that the misalignment problem has also been observed in attention training of speech recognition. Kim \etal 
%attributed the misalignment problem to the lack of left-to-right constraints as used in CTC, which is designed , and 
tried to solve the problem by using a joint CTC-attention model within the multi-task learning framework\cite{kim2016joint}. However, as pointed in \cite{cheng17fan}, the joint CTC-attention model does not work well in scene text reading.
%And it is theoretically unfeasible to attach a CTC decoder to the attention decoder by using the output of attention as the input of CTC, because the CTC decoding requires blanks between characters, which is not supported by attention model.
This paper also addresses the scene text recognition problem under the attention-based framework. Different from the existing methods, we propose a novel method EP that tries to estimate the probability of a string conditioned on the
%output \emph{pd} sequence
input image, by treating the misalignment between the $gt$ text and the output $pd$ sequence as the result of possible occurrences of missing/superfluous characters. EP provides an effective way to handle the misalignment problem, and empirically it outperforms the existing methods.
%{\color{red}give some words here to clarify the difference between EP and the CTC-attention model.}
